Predictive Biases in Natural Language Processing Models: A Conceptual Framework and Overview

An increasing number of works in natural language processing have addressed the effect of bias on the predicted outcomes, introducing mitigation techniques that act on different parts of the standard NLP pipeline (data and models). However, these works have been conducted in isolation, without a unifying framework to organize efforts within the field. This leads to repetitive approaches, and puts an undue focus on the effects of bias, rather than on their origins. Research focused on bias symptoms rather than the underlying origins could limit the development of effective countermeasures. In this paper, we propose a unifying conceptualization: the predictive bias framework for NLP. We summarize the NLP literature and propose a general mathematical definition of predictive bias in NLP along with a conceptual framework, differentiating four main origins of biases: label bias, selection bias, model overamplification, and semantic bias. We discuss how past work has countered each bias origin. Our framework serves to guide an introductory overview of predictive bias in NLP, integrating existing work into a single structure and opening avenues for future research.

==> todo.tex <==
\section*{TO BE REMOVED WHEN SUBMITTED}
ACL Reviews:

\url{https://docs.google.com/document/d/1wedxkFseWU00p1NBCp0ZFJy0f07-TmTAdvw_jkQTb2g/edit}

Bias Framework:
\url{https://docs.google.com/drawings/d/1c7RFPwGPmI2J_I5I2W-e2TSfdw-uOYYrmSn4AaHR24s/edit}

Appendix:
\url{https://www.overleaf.com/1837995922mwzcpnqntmrn}
\section*{TODOs}
\begin{itemize}
    
    \item add paragraph on source and target population (Andy) done

    \item add reasoning for ideal distribution for outcome disparity
    \begin{itemize}
        \item consider new name for ideal distribution
        \item add note about ideal distribution being subjective
    \end{itemize} -- Andy (start from response) done 
    
    \item add examples for the two types of disparities --Andy

    \item add reasoning for non-uniform distribution for error disparity
    \begin{itemize}
        \item contrast with outcome disparity 
        \item consider whether to rename error disparity to accuracy disparity and use an accuracy metric (leaning against)
        \item either way, explain decision of using error (i.e. because most optimization tries to minimize an error metric)
    \end{itemize} -- Andy (started from response)

    \item joint or conditional distribution in error disparity [Done: ]
    
    \item add structured steps (or developer process/algorithm/roadmap/workflow) on how to use framework to get rid of bias: 0. Specify target population and attributes of concern. 1. checking for consequence. If exists, check for potential origins; if potential origin exists, that doesn't necessarily mean potential origin is causing the disparity -- have to mitigate origin to see if it goes away. Mitigating the origin is often a context-specific. (examples -- stick to ones with papers: selection bias two common options: reweighting or resampling; label bias -- retrain annotators; mitigate during label aggregation -- remove biased annotators.) -- Deven [Done]
    
    \item make sure "ok" in gray scale
    
    \item check for syntax (newcite and cite) - Deven [Done.]
    
    \item write acknowledgements: Niranjan Balasubramanian, Lyle Ungar, Joao Sedoc, Salvatore Giorgi... 
    
    \item fix tense. 
    
    \item add explanation for semantic bias being not subsumed  (... it's within the latent space of the embeddings -- exists even without the pipeline: may or may not result in a disparity ...)
    
    \item move appendix separate -- Deven [Done]
    
    \item remove todo page
    
\end{itemize}

Dirk will submit 
